Training Overparametrized Neural Networks in Sublinear Time

The success of deep learning comes at a tremendous computational and energy cost, and the scalability of training massively overparametrized neural networks is becoming a real barrier to the progress of artificial intelligence (AI). Despite the popularity and low cost-per-iteration of traditional backpropagation via gradient decent, stochastic gradient descent (SGD) has prohibitive convergence rate in non-convex settings, both in theory and practice. To mitigate this cost, recent works have proposed to employ alternative (Newton-type) training methods with much faster convergence rate, albeit with higher cost-per-iteration. For a typical neural network with $m=\mathrm{poly}(n)$ parameters and input batch of $n$ datapoints in $\mathbb{R}^d$, the previous work of [Brand, Peng, Song, and Weinstein, ITCS'2021] requires $\sim mnd + n^3$ time per iteration. In this paper, we present a novel training method that requires only $m^{1-\alpha} n d + n^3$ amortized time in the same overparametrized regime, where $\alpha \in (0.01,1)$ is some fixed constant. This method relies on a new and alternative view of neural networks, as a set of binary search trees, where each iteration corresponds to modifying a small subset of the nodes in the tree. We believe this view would have further applications in the design and analysis of deep neural networks (DNNs).

==> app_miss_proof.tex <==
\section{Missing proofs for Section~\ref{sec:running_time}}
\label{sec:miss_proof}
Here in this section, we provide some missing proofs in Section~\ref{sec:running_time}. 

\begin{proof}[Proof of Lemma~\ref{lem:regression_time_formal}]
The algorithm calculate $R$ using $QR$ decomposition in line \ref{row:QR_decomposition} (Algorithm~\ref{alg:ours_formal}), which takes $O(n^3)$ time. 

We remark that, if we use $\mathsf{FMM}$, the running time is $O(n^\omega)$ \cite{w12}.

For the while-loop from line \ref{row:iterative_regression} (Algorithm~\ref{alg:ours_formal}), define $p$ as the iteration times of the while-loop from line \ref{row:iterative_regression} (Algorithm~\ref{alg:ours_formal}), then
\begin{align*}
p &= O(\log(1/\epsilon_{\text{reg}}))\\
&= O(\log (n/\lambda) ) \\
&= O(\log (\frac{n}{(\exp(-b^2/2)\cdot \frac{\delta}{100n^2})} ) )\\
&= O(\log (n/\delta) + b^2 )\\
&= O(\log (n/\delta) + \log m)\\
&= O(\log (n/\delta)),
\end{align*}
where the 1st step is from Corollary \ref{cor:iterative_regression}, the 2nd step is from line \ref{row:eps_reg} (Algorithm \ref{alg:ours_formal}), the 3rd step is from Theorem \ref{thm:sep}, the 4th step is from identical transformation, the 5th step is from $b= \Theta( \sqrt{\log m} )$
and the last step is from $\log m = O(\log n)$ since $m=\poly(n)$.

And in each iteration, note that $R$ is $n\times n$, $A$ is $md\times n$, $S$ is $t\times md$,
\begin{itemize}
\item we have calculating $v = R^\top A^\top (D \otimes I_d) A R z_t - R^\top y_{\mathrm{reg}}$ takes
\begin{align*}
    & ~ O(n^2 + o(mnd) + o(mnd) + n^2 + n^2) \\
    = & ~ O( o(mnd) +n^2)
\end{align*} 
time, 
\item and calculating $(R^\top A^\top (D \otimes I_d) A R)^\top v$ takes
\begin{align*}
    & ~ O(n^2+ o(mnd) + o(mnd) +n^2) \\
    = & ~ o(mnd) + O(n^2)
\end{align*}
time.
\end{itemize}
Thus let us consider each iteration in the while-loop from line \ref{row:iterative_regression} (Algorithm \ref{alg:ours_formal}), it will take $o(mnd)+O(n^2)$ time. Therefore, the total process of the iterative regression takes 
\begin{align*} 
O(( o(mnd) \log(n/\delta) + n^3)
\end{align*}
time.

We remark that, once we use $\mathsf{FMM}$, the it runs in 
\begin{align*} 
O( o(mnd) \log(n/\delta) + n^\omega).
\end{align*}
\end{proof}

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [Not Applicable]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

